Measuring the Significance of the Geographic Flow of Music

In previous work, our results suggested that some cities tend to be ahead of others in their musical preferences. We concluded that work by noting that to properly test this claim, we would try to exploit the leader-follower relationships that we identified to make predictions. Here we present the results of our predictive evaluation. We find that information on the past musical preferences in other cities allows a linear model to improve its predictions by approx. 5% over a simple baseline. This suggests that at best, previously found leader-follower relationships are rather weak.

==> intro.tex <==

In a recent paper, one of our results suggested that some cities may
systematically lead others in their musical preferences. \cite{Lee2012}
In that paper, we first came up with a test which, given a pair of
cities, should determine whether one city tends to follow the other. If
such a leader-follower relationship was found, then we created a
directed edge pointing from the follower to the leader. We observed that
when we looked at global structure of the graph produced in this manner,
it was nearly acyclic, as in \cref{fig:indie-flow}. Along the lines of
\cite{Nagy2010}, we interpreted the acyclic nature of the graph as
evidence that our results were meaningful, assuming that: (1) leadership
networks are expected to be highly acyclic, (2) if the pairwise
relationshisp we discovered were merely an artifact our our method, then
it is improbable that when combined in a global graph, that graph would
be acyclic, and (3) when we shuffled the data and applied our method, no
leader-follower relationships were detected.

\label{sec:flow}
\begin{figure}[h!]
  \centering
  \includegraphics[width=\columnwidth]{namerican_indie_p01}
  \caption{Example of a leader-follower network for the most active cities in
    Western Europe, as proposed in \cite{Lee2012}}
  \label{fig:indie-flow}
\end{figure}

However, we concluded that paper by noting that ``certain doubts remain,
and we should stress that our results reflect a work in progress...We
would be more confident of our results if we could demonstrate that the
model we create is meaninfgully predictive.'' Here we perform
experiments which check whether the types of relationships we
established in that previous work enable us to improve our predictions
of how musical preferences change.

We set up a prediction task where the goal of each estimator is to as
accurately as possible predict how the musical preferences in a target
city will change next week. For each prediction, the estimator is given
data on how music preferences changed in the past weeks in all cities
(including the target city itself). Each estimator is allowed to be
trained on approx. 2 years of years of data, and is then evaluated on
several months of a separate test dataset.  More details are presented
below.

If we were trying to predict what music will become more or less popular
in some target city, and we knew that the target city followed some
other leading city, then the history of that leading city should be
useful for predicting what will happen in the target city.  We find,
however, that when making these predictions, historical data from other
cities does not allow for meaningfully improved predictions for the
target city. In other words, the types of leader-follower relationships
we described in \cite{Lee2012} do not appear to be useful for making
predictions. This finding casts doubt on the meaninfulness of the
leader-follower relationships identified in \cite{Lee2012}.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

